A statistical study of propagating MHD kink waves in the quiescent corona

The Coronal Multi-channel Polarimeter (CoMP) has opened up exciting opportunities to probe transverse MHD waves in the Sun's corona. The archive of CoMP data is utilised to generate a catalogue of quiescent coronal loops that can be used for studying propagating kink waves. The catalogue contains 120 loops observed between 2012-2014. This catalogue is further used to undertake a statistical study of propagating kink waves in the quiet regions of the solar corona, investigating phase speeds, loop lengths, footpoint power ratio and equilibrium parameter values. The statistical study enables us to establish the presence of a relationship between the rate of damping and the length of the coronal loop, with longer coronal loops displaying weaker wave damping. We suggest the reason for this behaviour is related to a decreasing average density contrast between the loop and ambient plasma as loop length increases. The catalogue presented here will provide the community with the foundation for the further study of propagating kink waves in the quiet solar corona.

==> Statistical study of damping of propagating transverse waves in the solar corona/table_app.tex <==
\startlongtable
\begin{deluxetable*}{|c|c|c|c|c|c|c|c|}
\tablecaption{Measured loop parameters and wave parameters obtained from observations.\label{table01}}
%\tablewidth{600pt}
%\tabletypesize{5pt}
\tablehead{
\colhead{Loop no.} & 
\colhead{Solar-X} & 
\colhead{Solar-Y}& 
\colhead{Date} &
\colhead{Half Loop Length} &
\colhead{$\xi$} &
\colhead{Power Ratio} &  
\colhead{Phase speed}  \\ 
\colhead{} & 
\colhead{(arcsec)} &
\colhead{(arcsec)}  & 
\colhead{} &  
\colhead{(in Mm)} &
\colhead{} &
\colhead{} &
\colhead{(km s$^{-1}$)} 
} 
\startdata
       1 &       798.50 &      -819.50 & 20120423 &           42 &   -1.53 $\pm$ 1.27 &  2.1 $\pm$ 0.61 &    291 $\pm$ 2 \\ \hline
        2 &     -1026.30 &      -238.20 & 20120514 &           42 &   -8.04 $\pm$ 5.78 & 2.17 $\pm$ 0.72 &   415 $\pm$ 15 \\ \hline
        3 &       980.56 &       422.56 & 20120626 &           45 &   -0.95 $\pm$ 2.07 & 2.51 $\pm$ 1.07 &   561 $\pm$ 11 \\ \hline
        4 &      -928.26 &      -549.67 & 20120626 &           45 &    -1.89 $\pm$ 2.0 & 2.51 $\pm$ 1.07 &   561 $\pm$ 11 \\ \hline
        5 &     -1136.86 &       -57.01 & 20120410 &           55 &    2.49 $\pm$ 3.23 & 1.47 $\pm$ 0.63 &    373 $\pm$ 4 \\ \hline
        6 &     -1045.91 &      -251.79 & 20120514 &           58 &   -3.03 $\pm$ 1.64 &  2.0 $\pm$ 0.65 &   412 $\pm$ 15 \\ \hline
        7 &       504.41 &       944.64 & 20120410 &           58 &    5.28 $\pm$ 3.29 & 1.47 $\pm$ 0.63 &    373 $\pm$ 4 \\ \hline
        8 &       972.59 &       356.58 & 20120421 &           65 &   11.35 $\pm$ 5.55 & 0.86 $\pm$ 0.25 &   481 $\pm$ 11 \\ \hline
        9 &       911.23 &       553.31 & 20120719 &           65 &    1.88 $\pm$ 1.17 & 1.37 $\pm$ 0.58 &    402 $\pm$ 5 \\ \hline
       10 &     -1057.90 &        96.35 & 20120810 &           65 &  67.62 $\pm$ 30.86 & 1.38 $\pm$ 0.56 &    343 $\pm$ 6 \\ \hline
       11 &      1049.77 &      -168.19 & 20120121 &           71 &  24.04 $\pm$ 10.33 & 0.89 $\pm$ 0.33 &    376 $\pm$ 6 \\ \hline
       12 &     -1162.06 &       -39.82 & 20120410 &           78 &  24.06 $\pm$ 29.71 & 1.81 $\pm$ 0.78 &    512 $\pm$ 8 \\ \hline
       13 &       549.04 &      -918.78 & 20120410 &           81 &  50.13 $\pm$ 29.75 & 1.81 $\pm$ 0.78 &    512 $\pm$ 8 \\ \hline
       14 &      1098.97 &       124.52 & 20120626 &           81 &    1.74 $\pm$ 1.61 & 1.43 $\pm$ 0.61 &    389 $\pm$ 8 \\ \hline
       15 &      -883.66 &      -646.84 & 20120410 &           84 &   -3.74 $\pm$ 2.96 & 1.64 $\pm$ 0.71 &    365 $\pm$ 4 \\ \hline
       16 &       534.14 &       943.70 & 20120410 &           87 &   -1.87 $\pm$ 1.23 & 2.01 $\pm$ 0.87 &   566 $\pm$ 10 \\ \hline
       17 &     -1046.14 &       -52.13 & 20120410 &           87 &    -7.76 $\pm$ 3.1 & 1.64 $\pm$ 0.71 &    365 $\pm$ 4 \\ \hline
       18 &     -1052.56 &       214.08 & 20120423 &           87 &    2.65 $\pm$ 1.21 &  1.38 $\pm$ 0.4 &    300 $\pm$ 7 \\ \hline
       19 &      -343.39 &      1002.95 & 20120121 &           87 &    1.05 $\pm$ 0.59 & 0.58 $\pm$ 0.43 &   526 $\pm$ 10 \\ \hline
       20 &     -1055.64 &       -13.30 & 20120810 &           91 &  -17.92 $\pm$ 5.32 &  1.5 $\pm$ 0.61 &    308 $\pm$ 4 \\ \hline
       21 &       423.22 &     -1074.57 & 20130717 &           97 &    -2.0 $\pm$ 2.37 & 2.04 $\pm$ 0.88 &   630 $\pm$ 36 \\ \hline
       22 &      -628.86 &      -842.94 & 20120719 &           97 & -27.77 $\pm$ 11.13 & 1.71 $\pm$ 0.72 &    427 $\pm$ 6 \\ \hline
       23 &       925.44 &      -478.88 & 20130717 &          100 &  13.13 $\pm$ 13.96 & 1.49 $\pm$ 0.65 &    557 $\pm$ 9 \\ \hline
       24 &      -472.36 &      -967.83 & 20130717 &          100 &   26.27 $\pm$ 14.0 & 1.49 $\pm$ 0.65 &    557 $\pm$ 9 \\ \hline
       25 &     -1036.89 &      -204.53 & 20130717 &          100 &   -4.13 $\pm$ 2.58 & 2.04 $\pm$ 0.88 &   630 $\pm$ 36 \\ \hline
       26 &      -339.56 &      1007.43 & 20120121 &          103 &     3.1 $\pm$ 1.33 & 1.19 $\pm$ 0.44 &    537 $\pm$ 8 \\ \hline
       27 &      1028.62 &       357.55 & 20120719 &          107 &   -8.54 $\pm$ 2.71 &  1.7 $\pm$ 0.72 &    361 $\pm$ 7 \\ \hline
       28 &     -1052.56 &      -218.54 & 20130717 &          113 &   -6.06 $\pm$ 2.56 & 2.38 $\pm$ 1.03 &    489 $\pm$ 9 \\ \hline
       29 &       693.58 &      -833.45 & 20120410 &          113 &   15.42 $\pm$ 4.05 & 1.22 $\pm$ 0.52 &    315 $\pm$ 4 \\ \hline
       30 &       993.55 &       532.00 & 20120121 &          116 &     2.4 $\pm$ 0.92 & 0.77 $\pm$ 0.28 &   522 $\pm$ 15 \\ \hline
       31 &      1090.09 &        29.57 & 20120810 &          123 &   -7.75 $\pm$ 2.86 & 1.79 $\pm$ 0.74 &   512 $\pm$ 11 \\ \hline
       32 &      -935.88 &       549.79 & 20120410 &          123 &  45.25 $\pm$ 15.16 & 1.67 $\pm$ 0.72 &    439 $\pm$ 7 \\ \hline
       33 &      1111.05 &       -63.70 & 20120121 &          126 &    3.65 $\pm$ 0.53 & 0.45 $\pm$ 0.17 &    202 $\pm$ 5 \\ \hline
       34 &      -808.14 &      -692.31 & 20120410 &          126 &    8.26 $\pm$ 4.19 & 1.33 $\pm$ 0.57 &   675 $\pm$ 15 \\ \hline
       35 &      -647.63 &      -850.12 & 20120719 &          129 &   13.62 $\pm$ 3.91 & 1.33 $\pm$ 0.56 &    404 $\pm$ 5 \\ \hline
       36 &     -1050.43 &        80.15 & 20130717 &          129 &  53.42 $\pm$ 18.21 & 1.71 $\pm$ 0.75 &   461 $\pm$ 11 \\ \hline
       37 &      -983.72 &      -512.77 & 20120423 &          129 &    9.54 $\pm$ 4.12 & 1.42 $\pm$ 0.41 &    440 $\pm$ 8 \\ \hline
       38 &      -418.59 &      1004.38 & 20120121 &          129 &    -3.2 $\pm$ 1.33 &  1.61 $\pm$ 0.6 &   643 $\pm$ 11 \\ \hline
       39 &       737.25 &      -837.03 & 20120410 &          129 &    3.08 $\pm$ 1.57 &  0.94 $\pm$ 0.4 &   677 $\pm$ 15 \\ \hline
       40 &       623.30 &      -865.44 & 20120410 &          133 &  -11.43 $\pm$ 3.38 & 1.35 $\pm$ 0.58 &    415 $\pm$ 6 \\ \hline
       41 &       771.64 &      -726.14 & 20120423 &          133 &    2.91 $\pm$ 1.46 &  1.1 $\pm$ 0.32 &    515 $\pm$ 9 \\ \hline
       42 &     -1048.32 &        40.14 & 20120121 &          133 &  -18.39 $\pm$ 5.91 & 1.88 $\pm$ 0.69 &    537 $\pm$ 8 \\ \hline
       43 &     -1057.14 &      -255.49 & 20120514 &          133 &   -11.62 $\pm$ 2.6 & 1.76 $\pm$ 0.58 &   410 $\pm$ 13 \\ \hline
       44 &      1102.70 &      -207.84 & 20120121 &          142 &    2.03 $\pm$ 0.57 & 0.58 $\pm$ 0.22 &    445 $\pm$ 5 \\ \hline
       45 &      1029.24 &      -114.68 & 20120421 &          142 &    3.73 $\pm$ 0.96 & 0.72 $\pm$ 0.21 &   516 $\pm$ 28 \\ \hline
       46 &       830.82 &       774.90 & 20120810 &          146 &    4.11 $\pm$ 1.04 &  0.97 $\pm$ 0.4 &    402 $\pm$ 9 \\ \hline
       47 &       794.71 &       807.84 & 20120810 &          146 &    6.57 $\pm$ 1.56 & 1.25 $\pm$ 0.51 &    389 $\pm$ 6 \\ \hline
       48 &     -1054.36 &        48.97 & 20130717 &          149 &   -3.31 $\pm$ 0.94 & 2.09 $\pm$ 0.91 &    418 $\pm$ 9 \\ \hline
       49 &      -419.76 &      1012.89 & 20120121 &          155 &    2.09 $\pm$ 0.67 & 0.68 $\pm$ 0.25 &    587 $\pm$ 8 \\ \hline
       50 &      1098.00 &      -220.96 & 20120121 &          155 &   21.99 $\pm$ 5.02 & 1.59 $\pm$ 0.59 &    445 $\pm$ 6 \\ \hline
       51 &       566.20 &      -934.28 & 20120121 &          155 &    5.44 $\pm$ 1.73 &  0.83 $\pm$ 0.3 &   608 $\pm$ 11 \\ \hline
       52 &       628.47 &      -875.99 & 20120410 &          158 &  61.54 $\pm$ 14.87 & 1.36 $\pm$ 0.59 &    409 $\pm$ 6 \\ \hline
       53 &     -1063.02 &        22.18 & 20120120 &          158 &    7.42 $\pm$ 2.36 & 1.36 $\pm$ 0.57 &   549 $\pm$ 15 \\ \hline
       54 &      1116.94 &      -131.81 & 20140102 &          162 &   -25.26 $\pm$ 7.1 &  1.43 $\pm$ 0.6 &   499 $\pm$ 20 \\ \hline
       55 &      1139.13 &       203.94 & 20120121 &          162 &   34.77 $\pm$ 4.23 & 1.51 $\pm$ 0.56 &    246 $\pm$ 3 \\ \hline
       56 &       782.06 &      -736.51 & 20120423 &          171 &    1.73 $\pm$ 0.69 & 0.78 $\pm$ 0.23 &    507 $\pm$ 7 \\ \hline
       57 &      1094.88 &      -209.72 & 20120810 &          171 &   -7.86 $\pm$ 2.34 & 1.62 $\pm$ 0.66 &   577 $\pm$ 12 \\ \hline
       58 &       565.98 &      -942.74 & 20120121 &          171 &    9.31 $\pm$ 2.61 & 1.38 $\pm$ 0.51 &    598 $\pm$ 9 \\ \hline
       59 &      -951.82 &       557.94 & 20120410 &          175 &   -37.47 $\pm$ 7.9 & 1.45 $\pm$ 0.62 &    394 $\pm$ 6 \\ \hline
       60 &       638.63 &      -868.98 & 20120810 &          175 &   23.09 $\pm$ 8.19 & 1.22 $\pm$ 0.49 &   716 $\pm$ 22 \\ \hline
       61 &      1057.52 &       264.13 & 20120121 &          175 &   10.47 $\pm$ 2.08 & 0.95 $\pm$ 0.35 &   433 $\pm$ 10 \\ \hline
       62 &       758.52 &       724.19 & 20120719 &          175 &   24.02 $\pm$ 4.61 &  1.7 $\pm$ 0.73 &    362 $\pm$ 6 \\ \hline
       63 &      -958.90 &       561.96 & 20120410 &          184 & -109.0 $\pm$ 22.22 & 1.36 $\pm$ 0.58 &    405 $\pm$ 7 \\ \hline
       64 &       787.18 &      -744.80 & 20120423 &          184 & -99.76 $\pm$ 32.84 & 1.18 $\pm$ 0.34 &    485 $\pm$ 7 \\ \hline
       65 &      1072.37 &        74.36 & 20120719 &          184 & 141.25 $\pm$ 49.77 & 1.73 $\pm$ 0.73 &   717 $\pm$ 18 \\ \hline
       66 &      1066.31 &       397.09 & 20120421 &          191 &   17.88 $\pm$ 2.85 & 1.02 $\pm$ 0.29 &    473 $\pm$ 9 \\ \hline
       67 &     -1062.69 &         9.00 & 20120121 &          194 &   11.22 $\pm$ 2.23 & 0.74 $\pm$ 0.28 &    475 $\pm$ 8 \\ \hline
       68 &     -1080.66 &       119.18 & 20120423 &          197 &   23.79 $\pm$ 7.75 & 1.17 $\pm$ 0.33 &    511 $\pm$ 8 \\ \hline
       69 &      1034.72 &       361.26 & 20120421 &          197 &    5.36 $\pm$ 0.95 &  0.8 $\pm$ 0.23 &   501 $\pm$ 25 \\ \hline
       70 &     -1086.52 &        24.93 & 20120120 &          197 &  -33.08 $\pm$ 4.29 & 1.88 $\pm$ 0.79 &    285 $\pm$ 5 \\ \hline
       71 &      -974.84 &      -464.22 & 20120120 &          200 &    28.76 $\pm$ 6.5 & 1.21 $\pm$ 0.51 &   507 $\pm$ 17 \\ \hline
       72 &     -1093.16 &       -58.39 & 20120410 &          204 &   20.08 $\pm$ 3.71 & 1.19 $\pm$ 0.51 &    400 $\pm$ 7 \\ \hline
       73 &      -369.52 &      1028.94 & 20120121 &          204 &    12.7 $\pm$ 2.98 &  1.0 $\pm$ 0.37 &    589 $\pm$ 9 \\ \hline
       74 &     -1063.58 &       117.42 & 20130717 &          204 &   26.12 $\pm$ 5.55 & 1.46 $\pm$ 0.62 &   461 $\pm$ 12 \\ \hline
       75 &       564.80 &      -953.78 & 20120121 &          207 &    3.84 $\pm$ 0.98 & 0.64 $\pm$ 0.24 &   641 $\pm$ 13 \\ \hline
       76 &      -831.80 &      -722.20 & 20120410 &          210 &   10.15 $\pm$ 1.68 & 1.01 $\pm$ 0.43 &    365 $\pm$ 5 \\ \hline
       77 &      1127.22 &      -127.23 & 20120121 &          217 &   33.86 $\pm$ 4.64 & 1.07 $\pm$ 0.39 &    381 $\pm$ 4 \\ \hline
       78 &      -643.34 &      -879.80 & 20120719 &          217 &   25.83 $\pm$ 4.47 & 1.16 $\pm$ 0.48 &    414 $\pm$ 5 \\ \hline
       79 &      1058.06 &       359.66 & 20120421 &          217 &    5.81 $\pm$ 0.93 & 0.76 $\pm$ 0.22 &   501 $\pm$ 25 \\ \hline
       80 &       792.63 &      -769.79 & 20120423 &          223 &  -14.75 $\pm$ 3.96 & 1.32 $\pm$ 0.38 &    483 $\pm$ 8 \\ \hline
       81 &      1101.27 &       268.27 & 20120121 &          223 &    7.05 $\pm$ 0.78 & 0.61 $\pm$ 0.22 &    297 $\pm$ 6 \\ \hline
       82 &      1097.27 &       317.64 & 20120121 &          226 &    8.73 $\pm$ 1.28 & 0.73 $\pm$ 0.27 &    404 $\pm$ 7 \\ \hline
       83 &     -1149.07 &       -37.31 & 20120121 &          230 &   12.04 $\pm$ 1.84 & 0.97 $\pm$ 0.36 &    441 $\pm$ 6 \\ \hline
       84 &      1039.45 &       230.53 & 20120121 &          230 &     2.96 $\pm$ 0.6 &  0.53 $\pm$ 0.2 &   523 $\pm$ 15 \\ \hline
       85 &     -1045.10 &        97.27 & 20120423 &          233 &  -162.2 $\pm$ 45.2 & 1.27 $\pm$ 0.36 &   518 $\pm$ 11 \\ \hline
       86 &      1076.86 &       -84.21 & 20120421 &          239 &    7.48 $\pm$ 1.01 & 0.81 $\pm$ 0.23 &    486 $\pm$ 9 \\ \hline
       87 &     -1107.69 &        27.36 & 20120121 &          239 &  87.26 $\pm$ 14.96 & 1.15 $\pm$ 0.42 &    529 $\pm$ 8 \\ \hline
       88 &     -1137.79 &       -80.01 & 20120121 &          243 &    4.61 $\pm$ 0.69 & 0.53 $\pm$ 0.19 &    433 $\pm$ 7 \\ \hline
       89 &     -1059.30 &        89.12 & 20120423 &          246 &   37.74 $\pm$ 9.51 & 1.12 $\pm$ 0.32 &    492 $\pm$ 9 \\ \hline
       90 &      1133.61 &        29.86 & 20120719 &          249 &   10.73 $\pm$ 2.78 & 1.26 $\pm$ 0.53 &   699 $\pm$ 17 \\ \hline
       91 &      1094.80 &        76.04 & 20120719 &          252 &  -32.13 $\pm$ 6.69 & 1.53 $\pm$ 0.64 &   575 $\pm$ 16 \\ \hline
       92 &      -364.74 &      1059.90 & 20120121 &          255 &    9.64 $\pm$ 1.61 & 0.96 $\pm$ 0.35 &    531 $\pm$ 8 \\ \hline
       93 &       340.99 &      -998.73 & 20130717 &          265 &     9.4 $\pm$ 1.83 & 1.12 $\pm$ 0.49 &   528 $\pm$ 10 \\ \hline
       94 &     -1111.53 &       -73.92 & 20120410 &          272 & 298.17 $\pm$ 44.38 & 1.22 $\pm$ 0.52 &    436 $\pm$ 7 \\ \hline
       95 &      -861.38 &      -750.02 & 20120410 &          275 &   19.62 $\pm$ 2.79 & 0.99 $\pm$ 0.42 &    417 $\pm$ 5 \\ \hline
       96 &       583.79 &      -974.75 & 20120121 &          275 &    7.17 $\pm$ 1.41 & 1.04 $\pm$ 0.39 &   663 $\pm$ 12 \\ \hline
       97 &      1096.67 &       -67.21 & 20120421 &          275 &   11.61 $\pm$ 1.24 & 0.95 $\pm$ 0.27 &    448 $\pm$ 5 \\ \hline
       98 &       597.43 &      -975.40 & 20120121 &          281 &   54.77 $\pm$ 10.0 &  0.89 $\pm$ 0.3 &   653 $\pm$ 11 \\ \hline
       99 &       613.27 &      -918.13 & 20120810 &          281 &   20.03 $\pm$ 3.81 &  0.99 $\pm$ 0.4 &   619 $\pm$ 11 \\ \hline
      100 &     -1095.74 &        66.67 & 20120423 &          297 &    9.52 $\pm$ 1.96 & 0.96 $\pm$ 0.27 &    482 $\pm$ 7 \\ \hline
      101 &       559.78 &     -1031.05 & 20120121 &          297 &    3.67 $\pm$ 0.61 & 0.61 $\pm$ 0.22 &   593 $\pm$ 12 \\ \hline
      102 &      1030.30 &       206.40 & 20120121 &          314 &  -13.52 $\pm$ 1.79 & 1.17 $\pm$ 0.43 &   511 $\pm$ 17 \\ \hline
      103 &      1113.96 &       -63.69 & 20120421 &          317 &    7.43 $\pm$ 0.78 & 0.88 $\pm$ 0.26 &   488 $\pm$ 11 \\ \hline
      104 &       715.05 &      -781.73 & 20130410 &          320 &   15.01 $\pm$ 2.34 &  1.18 $\pm$ 0.5 &   532 $\pm$ 16 \\ \hline
      105 &       984.60 &      -432.80 & 20140102 &          327 &    70.0 $\pm$ 6.63 &  1.0 $\pm$ 0.42 &   338 $\pm$ 33 \\ \hline
      106 &     -1116.05 &        36.56 & 20120120 &          327 &   -16.65 $\pm$ 1.8 & 1.65 $\pm$ 0.69 &   388 $\pm$ 13 \\ \hline
      107 &      1131.76 &       -42.93 & 20120421 &          336 &    8.45 $\pm$ 0.83 & 0.85 $\pm$ 0.25 &   443 $\pm$ 43 \\ \hline
      108 &       906.47 &       552.07 & 20120719 &          340 &   57.12 $\pm$ 6.52 & 1.08 $\pm$ 0.45 &    428 $\pm$ 7 \\ \hline
      109 &      1135.61 &       100.60 & 20120719 &          349 &   21.41 $\pm$ 3.56 & 1.21 $\pm$ 0.51 &   632 $\pm$ 17 \\ \hline
      110 &       992.61 &       476.86 & 20120719 &          362 &   22.41 $\pm$ 2.43 &  0.96 $\pm$ 0.4 &    429 $\pm$ 6 \\ \hline
      111 &       935.90 &       647.84 & 20120810 &          365 & -102.21 $\pm$ 9.29 &  1.2 $\pm$ 0.49 &    388 $\pm$ 4 \\ \hline
      112 &     -1094.45 &       -56.87 & 20120121 &          417 &    9.39 $\pm$ 0.98 & 0.63 $\pm$ 0.24 &    530 $\pm$ 9 \\ \hline
      113 &       429.46 &     -1048.22 & 20130717 &          430 &   16.81 $\pm$ 1.96 & 0.97 $\pm$ 0.41 &   525 $\pm$ 11 \\ \hline
      114 &      -317.00 &      1032.62 & 20120120 &          453 &   19.62 $\pm$ 1.62 &  1.17 $\pm$ 0.5 &   403 $\pm$ 11 \\ \hline
      115 &      -666.95 &       794.06 & 20120514 &          466 &   -21.1 $\pm$ 1.35 & 2.61 $\pm$ 0.87 &   399 $\pm$ 11 \\ \hline
      116 &       912.78 &       532.07 & 20120719 &          475 &  116.17 $\pm$ 8.96 & 1.05 $\pm$ 0.44 &    407 $\pm$ 7 \\ \hline
      117 &      -322.68 &      1050.09 & 20120120 &          475 &  -15.88 $\pm$ 2.23 & 1.78 $\pm$ 0.76 &   738 $\pm$ 17 \\ \hline
      118 &       822.03 &      -708.55 & 20120423 &          479 &   11.75 $\pm$ 1.81 & 0.74 $\pm$ 0.22 &   567 $\pm$ 10 \\ \hline
      119 &       596.26 &      -935.79 & 20120120 &          524 &  -27.88 $\pm$ 2.64 &  1.67 $\pm$ 0.7 &   549 $\pm$ 15 \\ \hline
      120 &     -1077.38 &      -109.12 & 20120121 &          585 &    81.73 $\pm$ 5.7 &  1.36 $\pm$ 0.5 &    517 $\pm$ 9 \\ \hline
\enddata
\end{deluxetable*}
